Reinforcement Learning-Based Control for an Inline Skating Humanoid Robot

As humanoid robots become increasingly dynamic, coupling them with reinforcement learning offers a promising approach to solving the complex, underactuated mechanics of passive inline skating. Equipping a humanoid robot with passive inline skating wheels presents an opportunity to combine the versatile agility of humanoids with the high-speed, energy-efficient locomotion strategies utilized by human skaters. In this paper, we train and deploy a reinforcement learning control policy that enables novel locomotion strategies for a humanoid robot modified to equip consumer inline skates instead of conventional feet. Unlike previous work limited to quadrupedal robots or actively driven wheels, our system allows for precise 6-DoF control of the skates to execute dynamic, edge-driven propulsion strategies. Our skating strategies emerge entirely from our reward structure, without reliance on human motion data, imitation learning, or kinematic priors. We overcome the inherent instability of passive wheels and simulation contact artifacts by utilizing different geometric wheel models (spherical and ellipsoidal) during training and validation, along with a custom success-based command curriculum and a specialized rolling reward. Consequently, our policy demonstrates up to a 50% reduction in Cost of Transport (CoT) compared to standard walking gaits. The resulting policy successfully transfers zero-shot to the physical Booster T1 hardware. Real-world deployments demonstrate dynamic balance, the ability to reject active physical perturbations, and agile locomotion strategies capable of turning at speed. A video of our results can be found at https://www.youtube.com/watch?v=-_APcOS7uFo.

==> old_related_work.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \section{Related work} \label{related}

% Previous attempts to leverage the energy efficiency of skating with passive wheels in robotics have been largely limited to quadrupedal platforms that utilize specialized hardware modifications~\cite{Endo01052012}, such as high-friction claws to push off from~\cite{Bjelonic2018Skating}. Early foundational work in bipedal rollerblading explored specific mechanical designs and classical gait control generation~\cite{DesignGaitCastor}, but managing the inherent instability of single-line passive wheels remains a significant challenge, as it requires precise control over not only the position of the skates, but also the pitch, roll, and yaw angles of the wheels to properly engage the edges for propulsion and braking~\cite{skate_physics}, which requires 6 \ac{dof} for the skate end effector. These motions must be coordinated and depend on dynamic balancing, unlike actuated wheeled-legged systems that are able to propel themselves through mostly stable driving configurations~\cite{Bjelonic_2019}. Furthermore, the system faces significant partial observability; without encoders on the passive wheels, the controller must infer wheel speed and slippage through secondary sensors, complicating state estimation.

% To mitigate this instability, previous bipedal robots with unactuated wheels have often relied on conservative constraints. For example, some locomotion strategies completely avoid using a swing leg~\cite{Kimura2020}, keeping all passive wheels in continuous contact with the ground to maximize stability margins and prevent falls~\cite{zivSkate}. Although effective for basic movement, these approaches lack the dynamic robustness required to recover from perturbations or to execute complex locomotion behaviors such as human-like stroking, turning while accelerating, or rapid deceleration. Other skating robots have circumvented the difficulty of passive propulsion by using a combination of partially actuated and unactuated wheels, allowing the control policy to rely on simpler direct wheel actuation for straight forward acceleration~\cite{Disney2023StorytellingThroughCharactersSXSW}. In contrast to the above work, our approach aims to tackle the full complexity of passive skate control, utilizing friction and wheel edges for propulsion.

% Driven by advances in simulation environments, \ac{rl} has enabled humanoid robots to achieve high performance in complex whole body movement and control tasks such as martial arts~\cite{xie2025kungfubot} and table tennis~\cite{su2025hitterhumanoidtabletennis}. A parallel research topic, skateboarding humanoid robots, has also shown promising results using \ac{rl} control strategies. Previous control strategies utilizing precomputed open-loop motions~\cite{TaskasugiSkate} suffered from increasing complexity when attempting to incorporate turning while pushing and disturbances. However, training skateboarding control policies for humanoid robots in massively parallelizable simulation environments has proven feasible not only in simulation environments~\cite{Thibault2024LearningSkateboardingHumanoid}, but also with real-world deployment~\cite{han2026huskyhumanoidskateboardingphysicsaware}.

% Concurrent to our work, Gu et al.~\cite{Gu2026SKATER} recently introduced SKATER, a custom 25-DoF humanoid robot with integrated passive wheels designed specifically for roller skating. While their approach also utilizes a deep reinforcement learning framework and a multi-stage curriculum to achieve passive wheeled locomotion, their reward formulations; specifically inter-foot distance constraints and limb symmetry rewards, encourage the policy to converge on a continuous-contact "swizzle" gait where both feet remain on the ground. In contrast, our work tackles the integration of off-the-shelf consumer inline skates onto a general-purpose humanoid. Although our reward formulation incentivizes forward rolling, we impose no further structural priors on the emergent skating strategies. Furthermore, our decoupled wheel modeling technique successfully mitigates severe edge-angle artifacts, enabling a wider range of dynamic skating behaviors. 
